Optimality Conditions for Model Predictive Control: Rethinking Predictive Model Design

Optimality is a critical aspect of Model Predictive Control (MPC), especially in economic MPC. However, achieving optimality in MPC presents significant challenges, and may even be impossible, due to inherent inaccuracies in the predictive models. Predictive models often fail to accurately capture the true system dynamics, such as in the presence of stochasticity, leading to suboptimal MPC policies. In this paper, we establish the necessary and sufficient conditions on the underlying prediction model for an MPC scheme to achieve closed-loop optimality. Interestingly, these conditions are counterintuitive to the traditional approach of building predictive models that best fit the data. These conditions present a mathematical foundation for constructing models that are directly linked to the performance of the resulting MPC scheme.

==> acronyms.tex <==

\acrodef[SDM]{Sequential Decision Making}
% \begin{acronym}
    
%    \acro{mdp}[MDP]{Markov Decision Process}
%    \acro{rl}[RL]{Reinforcement Learning}
%    \acro{dp}[DP]{Dynamic Programming}
%    \acro{adp}[ADP]{Approximate Dynamic Programming}
%    \acro{sp}[SP]{Stochastic Programming}
%    \acro{lp}[LP]{Linear Programming}
%    \acro{mpc}[MPC]{Model Predictive Control}
%    \acro{empc}[EMPC]{Economic Model Predictive Control}
%    \acro{td}[TD]{Temporal Difference}
%    \acro{mbrl}[MBRL]{Model-based Reinforcement Learning}
%    \acro{dt}[DT]{Digital Twin}
%    \acro{ml}[ML]{Machine Learning}
%    \acro{lstm}[LSTM]{Long Short-Term Memory}
%    \acro{rnn}[RNN]{Recurrent Neural Network }
%    \acro{dnn}[DNN]{Deep Neural Network }
%    \acro{dnns}[DNNs]{Deep Neural Networks}
%    \acro{gp}[GP]{Gaussian Processes}
%    \acro{ai}[AI]{Artificial Intelligence}
%    \acro{mle}[MLE]{Maximum Likelihood Estimation}
%    \acro{lqr}[LQR]{Linear Quadratic Regulator}
%    \acro{gpu}[GPU]{Graphics processing unit}
%    \acro{tpu}[TPU]{Tensor processing unit}
%    \acro{gans}[GANs]{Generative Adversarial Networks}
%    \acro{cnns}[CNNs]{Convolutional Neural Networks}
%    \acro{ls}[LS]{Least Squares}
%    \acro{mse}[MSE]{Mean Squared Error}
%     \acro{map}[MAP]{Maximum A Posteriori}
%     \acro{gmm}[GMM]{Gaussian Mixture Model}
%     \acro{hmm}[HMM]{Hidden Markov Model}
%     \acro{elbo}[ELBO]{Evidence Lower Bound}
%     \acro{vae}[VAE]{Variational Autoencoder}
%     \acro{gan}[GAN]{Generative Adversarial Network}
%     \acro{ode}[ODE]{Ordinary Differential Equations}
%     \acro{ude}[UDE]{Universal Differential Equations} 
%     \acro{ham}[HAM]{Hybrid Analysis and Modeling} 
%     \acro{vi}[VI]{Variational Inference} 
%     \acro{em}[EM]{Expectation-Maximization} 
%     \acro{lstdq}[LSTDQ]{Least Square Temporal Difference Q-learning} 
% \end{acronym}


